FinBERT-QA: Financial Question Answering with pre-trained BERT Language Models

Motivated by the emerging demand in the financial industry for the automatic analysis of unstructured and structured data at scale, Question Answering (QA) systems can provide lucrative and competitive advantages to companies by facilitating the decision making of financial advisers. Consequently, we propose a novel financial QA system using the transformer-based pre-trained BERT language model to address the limitations of data scarcity and language specificity in the financial domain. Our system focuses on financial non-factoid answer selection, which retrieves a set of passage-level texts and selects the most relevant as the answer. To increase efficiency, we formulate the answer selection task as a re-ranking problem, in which our system consists of an Answer Retriever using BM25, a simple information retrieval approach, to first return a list of candidate answers, and an Answer Re-ranker built with variants of pre-trained BERT language models to re-rank and select the most relevant answers. We investigate various learning, further pre-training, and fine-tuning approaches for BERT. Our experiments suggest that FinBERT-QA, a model built from applying the Transfer and Adapt further fine-tuning and pointwise learning approach, is the most effective, improving the state-of-the-art results of task 2 of the FiQA dataset by 16% on MRR, 17% on NDCG, and 21% on Precision@1.

==> algorithms/forwardRNN.tex <==
\begin{algorithm}[p]
\caption{Forward RNN}
\label{alg:forwardRNN}
\begin{algorithmic}
    % \ttfamily
    \State Returns output sequence $y$
    \State $h_{0} \gets 0$
    \ForEach{$\vec{i} \gets \vec{1}$ to \textsc{length}(x)}
        \State $\vec{h}_{\vec{i}} \gets g(U \; h_{i-1} + W \; x_{i})$  
      \State $\vec{y}_{\vec{i}} \gets f(V \; h_{i})$  
 
    \EndFor \\
    \Return $y$
\end{algorithmic}
\end{algorithm}

==> chapters/0_2-abstract.tex <==
\chapter{Abstract}
foo bar

==> chapters/1-introduction.tex <==
\chapter{Introduction}\label{chap:introduction}
This is a template for an undergraduate or master's thesis.
The first sections are concerned with the template itself. If this is your first
thesis, consider reading \secref{sec:advice}.

Of course, the structure of this
thesis is only an example.
Discuss with your adviser what structure fits best for your thesis.

\section{Template Structure}
\begin{itemize}
    \item To compile the document either run the makefile or run your compiler on the file `thesis\_main.tex'. The included makefile requires latexmk which automatically runs bibtex and recompiles your thesis as often as needed. Also it automatically places all output files (aux, bbl, ...) in the folder `out'. As the pdf also goes in there, the makefile copies the pdf file to the parent folder. There is also a makefile in the chapters folder, to ensure you can also compile from this directory.

    \item The file `setup.tex' includes the packages and defines commands. For more details see \secref{sec:setup}.

    \item Each chapter goes into a separate document, the files can be found in the folder chapters.

    \item The bib folder contains the .bib files, I'd suggest to create multiple bib files for different topics. If you add some or rename the existing ones, don't forget to also change this in thesis\_main.tex. You can then cite as usual~\cite{kingma2014adam, bromley1993siamesesignature,muja2009flann}.

    \item The template is written in a way that eases the switch from scrbook to book class. So if you're not a fan of KOMA you can just replace the documentclass in the main file. The only thing that needs to be changed in setup.tex is the caption styling, see the comments there.
\end{itemize}


\section{setup.tex}\label{sec:setup}
Edit setup.tex according to your needs. The file contains two sections, one for package includes, and one for defining commands. At the end of the includes and commands there is a section that can safely be removed if you don't need algorithms or tikz. Also don't forget to adapt the pdf hypersetup!!\\
setup.tex defines:
\begin{itemize}
    \item some new commands for remembering to do stuff:
    \begin{itemize}
        \item \verb|\todo{Do this!}|: \todo{Do this!}
        \item \verb|\extend{Write more when new results are out!}|:\\ \extend{Write more when new results are out!}
        \item \verb|\draft{Hacky text!}|: \draft{Hacky text!}
    \end{itemize}

    \item some commands for referencing, `in \verb|\chapref{chap:introduction}|' produces 'in \chapref{chap:introduction}'
    \begin{itemize}
        \item \verb|\chapref{}|
        \item \verb|\secref{sec:XY}|
        \item \verb|\eqref{}|
        \item \verb|\figref{}|
        \item \verb|\tabref{}|
    \end{itemize}

    \item the colors of the Uni's corporate design, accessible with\\ \verb|{\color{UniX} Colored Text}|
    \begin{itemize}
        \item {\color{UniBlue}UniBlue}
        \item {\color{UniRed}UniRed}
        \item {\color{UniGrey}UniGrey}
    \end{itemize}

    \item a command for naming matrices \verb|\mat{G}|, $\mat{G}$, and naming vectors \verb|\vec{a}|, $\vec{a}$. This overwrites the default behavior of having an arrow over vectors, sticking to the naming conventions  normal font for scalars, bold-lowercase for vectors, and bold-uppercase for matrices.

    \item named equations:
        \begin{verbatim}
\begin{align}
    d(a,b) &= d(b,a)\\ \eqname{symmetry}
\end{align}
        \end{verbatim}
        \begin{align}
            d(a,b) &= d(b,a)\\ \eqname{symmetry}
        \end{align}
\end{itemize}

\section{Advice}\label{sec:advice}
This section gives some advice how to write a thesis ranging from writing style to formatting. To be sure, ask your advisor about his/her preferences.\\
For a more complete list we recommend to read Donald Knuth's paper on mathematical writing. (At least the first paragraph). \url{http://jmlr.csail.mit.edu/reviewing-papers/knuth_mathematical_writing.pdf}

    \begin{itemize}

        \item If you use formulae pay close attention to be consistent throughout the thesis!

        \item Usually  in a thesis you don't write `In [24] the data is..'. You have more space than a paper has, so write `AuthorXY et al. prepare the data... [24]'. Also pay attention to the placement: The citation is at the end of the sentence before the full stop with a no-break space. \verb|... last word~\cite{XY}.|

        \item Pay attention to comma usage, there is a big difference between English and German. `...the fact that bla...' etc.

        \item Do not write `don't ', `can't' etc. Write `do not', `can not'.

        \item If an equation is at the end of a sentence, add a full stop. If it's not the end, add a comma: {$a= b + c$~~~~(1),}

        \item Avoid footnotes if possible.

        \item Use \verb|``''| for citing, not \verb|""|.

        \item It's important to look for spelling mistakes in your thesis. There are also tools like aspell that can help you find such mistakes.
        This is never an excuse not to properly read your thesis again, but it can help.
        You can find an introduction under \url{https://git.fachschaft.tf/fachschaft/aspell}.

        \item If have things like a graph or any other drawings consider using tikz, if you need function graphs or diagrams consider using pgfplots.
        This has the advantage that the style will be more consistent (same font, formatting options etc.) than when you use some external program.

        \item Discuss with your advisor whether to use passive voice or not. In most computer science papers passive voice is avoided. It's harder to read, more likely to produce errors, and most of the times less precise. Of course there are situations where the passive voice fits but in scientific papers they are rare. Compare the sentence: `We created the wheel to solve this.' to `The wheel was created to solve this', you don't know who did it, making it harder to understand what is your contribution and what is not.
        
        \item In tables avoid vertical lines, keep them clean and neat. See \ref{tab:accuracy} for an example. More details can be found in the `Small Guide to Making Nice Tables' \url{https://www.inf.ethz.ch/personal/markusp/teaching/guides/guide-tables.pdf}

    \end{itemize}


==> chapters/2-relatedwork.tex <==
\chapter{Related Work}\label{chap:relatedwork}
Give a brief overview of the work relevant for your thesis. 

==> chapters/3-background.tex <==
\chapter{Background}\label{chap:background}
Explain the math and notation.

==> chapters/4-approach.tex <==
\chapter{Approach}\label{chap:approach}
The approach usually starts with the problem definition and continues with what you have done. Try to give an intuition first and describe everything with words and then be more formal like `Let $g$ be ...'.

\section{Problem Definition}
Start with a very short motivation why this is important. Then, as stated above, describe the problem with words before getting formal.

\section{First Part of the Approach}

\section{N-th Part of the Approach}

==> chapters/5-experiments.tex <==
\chapter{Experiments}\label{chap:experiments}



==> chapters/6-conclusions.tex <==
\chapter{Conclusion}\label{chap:conclusion}

==> chapters/7-acknowledgments.tex <==
\chapter{Acknowledgments}

I would like to thank:

\begin{itemize}
\item Dr. Fang Wei-Kleiner for providing me the freedom and encouragement to explore a topic of my interest for my thesis. I am sincerely grateful for her feedback and  motivating advice. 
\item Prof. Dr. Josif Grabocka for agreeing to be my second examiner.
\item Dogu Araci, the creator of FinBERT, for the inspiration of my thesis as well as for his support for helping me understand the theoretical concepts of BERT.
\item My proofreaders:
\item My mother for the motivation and support.
\item My friend Marina Roth for always being there for me and encouraging me throughout my thesis and course of studies.
\end{itemize}

